ARO-Net: Learning Implicit Fields from Anchored Radial Observations

We introduce anchored radial observations (ARO), a novel shape encoding for learning implicit field representation of 3D shapes that is category-agnostic and generalizable amid significant shape variations. The main idea behind our work is to reason about shapes through partial observations from a set of viewpoints, called anchors. We develop a general and unified shape representation by employing a fixed set of anchors, via Fibonacci sampling, and designing a coordinate-based deep neural network to predict the occupancy value of a query point in space. Differently from prior neural implicit models that use global shape feature, our shape encoder operates on contextual, query-specific features. To predict point occupancy, locally observed shape information from the perspective of the anchors surrounding the input query point are encoded and aggregated through an attention module, before implicit decoding is performed. We demonstrate the quality and generality of our network, coined ARO-Net, on surface reconstruction from sparse point clouds, with tests on novel and unseen object categories, "one-shape" training, and comparisons to state-of-the-art neural and classical methods for reconstruction and tessellation.

==> figures/ablation_anchors.tex <==
\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/anchor_ablation.pdf}
  \caption{How different anchor placement strategies affect network performance, where anchor count $m = 48$ for all settings.}
  \label{fig:anchor_ablation}
\end{figure}

==> figures/eval_qual_anchor_sampling.tex <==
\begin{figure*}
\centering
  \includegraphics[width=\textwidth]{images/eval_qual_anchor_sampling.png}
  \caption{Visual comparisons among different anchor placement strategies. Zoom-ins highlight the reconstruction difference among three strategies.}
  \label{fig:eval_qual_anchor_sampling}
\end{figure*}

==> figures/full_cover.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.99\linewidth]{images/full_cover2.pdf}
%\caption{Visualization of ARO-Net activation, trained on a single letter ``G`` and tested on ``P``. 

\label{fig:cover}
\end{figure}


==> figures/single_shape_2d_comp.tex <==
\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/single_shape_2d_comp.png}
  \caption{Reconstructing other letters when trained only on `R'. The blue points are anchors and they can only observe the red contours of letters.}
  \label{fig:single_shape_2d_comp}
\end{figure}

==> figures/single_shape_overfit.tex <==
\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/overfit_sphere.png}
  \caption{Training on a sphere but testing on a cube.}
  \label{fig:single_shape_3d_comp}
\end{figure}
% Reconstructing a cube when the network overfits a sphere.

==> figures/tab_ARONet_output.tex <==
\begin{table}
	\centering
	\caption{Effect of the network's output.}
	\begin{tabular}{lcccc}
		\toprule
		Training & MC & CD & Norm & OCC\\
		\midrule
         occ  & occ & 1.50  & 9.13 & 9.133  \\
         dist  & dist  &   &   &  \\
         occ+dist & dist  & 1.86  & 0.92 & 9.040  \\
         occ+dist & occ & 1.91  &  9.13 & 9.136 \\

		\bottomrule
	\end{tabular}
    \label{tab:ARONet_output}
\end{table}	

==> figures/tab_diff_num_of_points.tex <==
\begin{table}
	\centering
	\caption{Parameter and ablation study. Experiments were conducted on ABC.}
	\resizebox{.99\columnwidth}{!}{
	\begin{tabular}{lrrrrrrr}
		\toprule
		$n$ & & Method & LFD$\downarrow$ & HD$\downarrow$ & CD$\downarrow$  & EMD$\downarrow$  & OCC$\uparrow$ \\
		\midrule

         $n=512$ & P2S &  &   &  8.70   & & 8.16 \\
         $n=512$ & UNDC & 2.11 &   &  8.70   & & 8.16 \\
         $n=512$ & ARO-Net & 1.98 &   &  8.70   & & 8.16 \\
         $n=1024$ &  &    &  &  &  \\
         $n=1024$ &  &    &  &  &  \\
         $n=1024$ &  &    &  &  &  \\
         $n=2048$ &  &    &  &  &  \\
         $n=2048$ &  &    &  &  &  \\
         $n=2048$ &  &    &  &  &  \\
         Default &  &    &  &  & \\
		\bottomrule
	\end{tabular}
	}
    \label{tab:param_and_ablation}
\end{table}	

==> figures/trained_on_big_r.tex <==
\begin{figure}
\centering
  \includegraphics[width=\columnwidth]{images/trained_on_R.pdf}
  \caption{2D version of ARO-Net trained on `R's and tested on other glyphs. Blue points denote the anchors, and red contours denote visible boundaries from these anchors.}
  \label{fig:trained_on_big_r}
\end{figure}
